Mozualization: Crafting Music and Visual Representation with Multimodal AI

In this work, we introduce Mozualization, a music generation and editing tool that creates multi-style embedded music by integrating diverse inputs, such as keywords, images, and sound clips (e.g., segments from various pieces of music or even a playful cat's meow). Our work is inspired by the ways people express their emotions -- writing mood-descriptive poems or articles, creating drawings with warm or cool tones, or listening to sad or uplifting music. Building on this concept, we developed a tool that transforms these emotional expressions into a cohesive and expressive song, allowing users to seamlessly incorporate their unique preferences and inspirations. To evaluate the tool and, more importantly, gather insights for its improvement, we conducted a user study involving nine music enthusiasts. The study assessed user experience, engagement, and the impact of interacting with and listening to the generated music.

==> Tables/CompletionTime_Novice.tex <==
% \begin{table}[h]
\centering
% \label{tab:CompletionTime_Novice}
\begin{tabular}{@{}>{\centering\arraybackslash}m{3cm}cccccc@{}} 
\toprule
\multirow{2}{*}[-0.5ex]{Condition} & \multicolumn{2}{c}{Curve Brushing} & \multicolumn{2}{c}{Object Manipulation} \\ \cmidrule(l){2-3} \cmidrule(l){4-5} 
                          & Effect Size   & CI  & Effect Size   & CI  \\ \midrule
D+D                       &27.808s          &[23.869, 32.398]             &22.520s          &[19.864, 25.530]             \\
I+D                       &25.074s          &[21.894, 28.717]             &19.523s          &[17.025, 22.388]             \\
F+D                       &21.887s          &[18.783, 25.503]             &20.453s          &[17.565, 23.816]             \\
D+I                       &29.753s          &[26.080, 33.945]             &26.240s          &[22.961, 29.988]             \\
I+I                       &26.589s          &[22.870, 30.913]             &23.288s          &[20.419, 26.559]             \\
F+I                       &27.188s          &[23.961, 30.850]             &23.775s          &[20.964, 26.963]             \\ \bottomrule
\end{tabular}
% \caption{The mean task completion times and their corresponding 95\% confidence intervals of novices.}
% \end{table}

==> Tables/CompletionTime_VRuser.tex <==
% \begin{table}[h]
\centering
% \label{tab:CompletionTime_VRuser}
\begin{tabular}{@{}>{\centering\arraybackslash}m{3cm}cccccc@{}} 
\toprule
\multirow{2}{*}[-0.5ex]{Condition} & \multicolumn{2}{c}{Curve Brushing} & \multicolumn{2}{c}{Object Manipulation} \\ \cmidrule(l){2-3} \cmidrule(l){4-5} 
                          & Effect Size   & CI  & Effect Size   & CI  \\ \midrule
D+D                       &27.488s          &[23.811, 31.733]             &24.379s          &[20.950, 28.370]             \\
I+D                       &25.362s          &[22.849, 28.152]             &22.874s          &[19.583, 26.717]             \\
F+D                       &23.755s          &[21.063, 26.792]             &21.922s          &[18.449, 26.048]             \\
D+I                       &29.373s          &[26.128, 33.022]             &23.308s          &[19.736, 27.526]             \\
I+I                       &29.413s          &[26.389, 32.783]             &27.125s          &[23.538, 31.258]             \\
F+I                       &26.677s          &[23.901, 29.775]             &22.740s          &[19.059, 27.132]             \\ \bottomrule
\end{tabular}
% \caption{The mean task completion times and their corresponding 95\% confidence intervals of VR users.}
% \end{table}

==> Tables/CompletionTime_all.tex <==
% \begin{table}[h]
\centering
% \label{tab:CompletionTime_all}
\begin{tabular}{@{}>{\centering\arraybackslash}m{3cm}cccccc@{}} 
\toprule
\multirow{2}{*}[-0.5ex]{Condition} & \multicolumn{2}{c}{Curve Brushing} & \multicolumn{2}{c}{Object Manipulation} \\ \cmidrule(l){2-3} \cmidrule(l){4-5} 
                          & Effect Size   & CI  & Effect Size   & CI  \\ \midrule
D+D                       &27.661s          &[24.933, 30.688]             &23.354s          &[21.222, 25.700]             \\
I+D                       &25.206s          &[23.125, 27.474]             &20.993s          &[18.954, 23.251]             \\
F+D                       &22.724s          &[20.601, 25.067]             &21.114s          &[18.870, 23.624]             \\
D+I                       &29.578s          &[27.094, 32.291]             &24.853s          &[22.402, 27.571]             \\
I+I                       &27.848s          &[25.337, 30.607]             &24.974s          &[22.690, 27.488]             \\
F+I                       &26.953s          &[24.794, 29.300]             &23.295s          &[20.997, 25.845]             \\ \bottomrule
\end{tabular}
% \caption{The mean task completion times and their corresponding 95\% confidence intervals of all participants.}
% \end{table}

==> Tables/ErrorAmount_Novice.tex <==
% \begin{table}[h]
\centering
% \label{tab:ErrorAmount_novice}
\begin{tabular}{@{}>{\centering\arraybackslash}m{3cm}cccccc@{}} 
\toprule
\multirow{2}{*}[-0.5ex]{Condition} & \multicolumn{2}{c}{Curve Brushing} & \multicolumn{2}{c}{Object Manipulation} \\ \cmidrule(l){2-3} \cmidrule(l){4-5} 
                          & Effect Size   & CI  & Effect Size   & CI  \\ \midrule
D+D                       &.700cm          &[.635, .790]             &.141cm          &[.112, .176]             \\
I+D                       &.682cm          &[.630, .743]             &.134cm          &[.114, .158]             \\
F+D                       &.723cm          &[.650, .811]             &.138cm          &[.111, .173]             \\
D+I                       &.782cm          &[.711, .868]             &.171cm          &[.130, .239]             \\
I+I                       &.814cm          &[.737, .932]             &.202cm          &[.158, .256]             \\
F+I                       &.792cm          &[.713, .887]             &.205cm          &[.168, .252]             \\ \bottomrule
\end{tabular}
% \caption{The mean task error amounts in cm and their corresponding 95\% confidence intervals of novices.}
% \end{table}

==> Tables/ErrorAmount_VRuser.tex <==
% \begin{table}[h]
\centering
% \label{tab:ErrorAmount_VRuser}
\begin{tabular}{@{}>{\centering\arraybackslash}m{3cm}cccccc@{}} 
\toprule
\multirow{2}{*}[-0.5ex]{Condition} & \multicolumn{2}{c}{Curve Brushing} & \multicolumn{2}{c}{Object Manipulation} \\ \cmidrule(l){2-3} \cmidrule(l){4-5} 
                          & Effect Size   & CI  & Effect Size   & CI  \\ \midrule
D+D                       &.595cm          &[.545, .656]             &.111cm          &[.091, .135]             \\
I+D                       &.550cm          &[.518, .590]             &.098cm          &[.079, .126]             \\
F+D                       &.556cm          &[.520, .599]             &.148cm          &[.119, .185]             \\
D+I                       &.624cm          &[.588, .665]             &.116cm          &[.092, .152]             \\
I+I                       &.723cm          &[.655, .839]             &.175cm          &[.146, .207]             \\
F+I                       &.638cm          &[.594, .684]             &.191cm          &[.157, .234]             \\ \bottomrule
\end{tabular}
% \caption{The mean task error amounts in cm and their corresponding 95\% confidence intervals of VR users.}
% \end{table}

==> Tables/ErrorAmount_all.tex <==
% \begin{table}[h]
\centering
% \label{tab:ErrorAmount_all}
\begin{tabular}{@{}>{\centering\arraybackslash}m{3cm}cccccc@{}} 
\toprule
\multirow{2}{*}[-0.5ex]{Condition} & \multicolumn{2}{c}{Curve Brushing} & \multicolumn{2}{c}{Object Manipulation} \\ \cmidrule(l){2-3} \cmidrule(l){4-5} 
                          & Effect Size   & CI  & Effect Size   & CI  \\ \midrule
D+D                       &.652cm          &[.608, .706]             &.127cm          &[.109, .150]             \\
I+D                       &.622cm          &[.587, .662]             &.118cm          &[.103, .135]             \\
F+D                       &.647cm          &[.604, .707]             &.143cm          &[.122, .166]             \\
D+I                       &.710cm          &[.666, .764]             &.146cm          &[.120, .185]             \\
I+I                       &.772cm          &[.714, .848]             &.189cm          &[.163, .223]             \\
F+I                       &.722cm          &[.674, .780]             &.198cm          &[.172, .229]             \\ \bottomrule
\end{tabular}
% \caption{The mean task error amounts in cm and their corresponding 95\% confidence intervals of all participants.}
% \end{table}

==> Tables/PreferenceRating_Novice.tex <==
% \begin{table}[h]
\centering
% \label{tab:ErrorAmount_novice}
\begin{tabular}{@{}>{\centering\arraybackslash}m{3cm}cccccc@{}} 
\toprule
\multirow{2}{*}[-0.5ex]{Condition} & \multicolumn{2}{c}{Curve Brushing} & \multicolumn{2}{c}{Object Manipulation} \\ \cmidrule(l){2-3} \cmidrule(l){4-5} 
                          & Effect Size   & CI  & Effect Size   & CI  \\ \midrule
D+D                       &3.000          &[2.231, 3.769]             &3.615          &[2.538, 4.615]             \\
I+D                       &4.385          &[3.385, 5.077]             &5.000          &[4.385, 5.462]             \\
F+D                       &5.077          &[4.154, 5.692]             &4.462          &[3.385, 5.077]             \\
D+I                       &2.769          &[2.231, 3.231]             &2.077          &[1.615, 2.615]             \\
I+I                       &2.462          &[1.615, 3.615]             &2.692          &[1.846, 3.692]             \\
F+I                       &3.308          &[2.538, 4.000]             &3.154          &[2.615, 3.846]             \\ \bottomrule
\end{tabular}
% \caption{The mean condition preference rating (obtained by rank conversion) and their corresponding 95\% confidence intervals of novices.}
% \end{table}

==> Tables/PreferenceRating_VRuser.tex <==
% \begin{table}[h]
\centering
% \label{tab:ErrorAmount_VRuser}
\begin{tabular}{@{}>{\centering\arraybackslash}m{3cm}cccccc@{}} 
\toprule
\multirow{2}{*}[-0.5ex]{Condition} & \multicolumn{2}{c}{Curve Brushing} & \multicolumn{2}{c}{Object Manipulation} \\ \cmidrule(l){2-3} \cmidrule(l){4-5} 
                          & Effect Size   & CI  & Effect Size   & CI  \\ \midrule
D+D                       &3.364          &[2.545, 4.364]             &3.818          &[2.636, 4.818]             \\
I+D                       &4.909          &[4.091, 5.545]             &5.455          &[5.000, 5.818]             \\
F+D                       &4.636          &[3.727, 5.364]             &3.909          &[3.182, 4.727]             \\
D+I                       &2.364          &[1.636, 3.273]             &2.364          &[1.727, 3.182]             \\
I+I                       &2.909          &[2.182, 3.727]             &2.818          &[2.000, 3.727]             \\
F+I                       &2.818          &[1.909, 3.727]             &2.636          &[1.909, 3.364]             \\ \bottomrule
\end{tabular}
% \caption{The mean condition preference rating (obtained by rank conversion) and their corresponding 95\% confidence intervals of VR users.}
% \end{table}

==> Tables/PreferenceRating_all.tex <==
% \begin{table}[h]
\centering
% \label{tab:ErrorAmount_all}
\begin{tabular}{@{}>{\centering\arraybackslash}m{3cm}cccccc@{}} 
\toprule
\multirow{2}{*}[-0.5ex]{Condition} & \multicolumn{2}{c}{Curve Brushing} & \multicolumn{2}{c}{Object Manipulation} \\ \cmidrule(l){2-3} \cmidrule(l){4-5} 
                          & Effect Size   & CI  & Effect Size   & CI  \\ \midrule
D+D                       &3.167          &[2.583, 3.792]             &3.708          &[2.958, 4.417]             \\
I+D                       &4.625          &[3.958, 5.125]             &5.208          &[4.833, 5.500]             \\
F+D                       &4.875          &[4.250, 5.375]             &4.208          &[3.583, 4.708]             \\
D+I                       &2.583          &[2.125, 3.042]             &2.208          &[1.833, 2.667]             \\
I+I                       &2.667          &[2.042, 3.375]             &2.750          &[2.167, 3.417]             \\
F+I                       &3.083          &[2.500, 3.667]             &2.917          &[2.458, 3.458]             \\ \bottomrule
\end{tabular}
% \caption{The mean condition preference rating (obtained by rank conversion) and their corresponding 95\% confidence intervals of all participants.}
% \end{table}
